Towards Collaborative Drilling with a Cobot Using Admittance Controller

In the near future, collaborative robots (cobots) are expected to play a vital role in the manufacturing and automation sectors. It is predicted that workers will work side by side in collaboration with cobots to surpass fully automated factories. In this regard, physical human-robot interaction (pHRI) aims to develop natural communication between the partners to bring speed, flexibility, and ergonomics to the execution of complex manufacturing tasks. One challenge in pHRI is to design an optimal interaction controller to balance the limitations introduced by the contradicting nature of transparency and stability requirements. In this paper, a general methodology to design an admittance controller for a pHRI system is developed by considering the stability and transparency objectives. In our approach, collaborative robot constrains the movement of human operator to help with a pHRI task while an augmented reality (AR) interface informs the operator about its phases. To this end, dynamical characterization of the collaborative robot (LBR IIWA 7 R800, KUKA Inc.) is presented first. Then, the stability and transparency analyses for our pHRI task involving collaborative drilling with this robot are reported. A range of allowable parameters for the admittance controller is determined by superimposing the stability and transparency graphs. Finally, three different sets of parameters are selected from the allowable range and the effect of admittance controllers utilizing these parameter sets on the task performance is investigated.

==> procedure.tex <==
\section{Procedure}

In the controller parameter space, which corresponds to all possible combinations of controller parameters that are studied, the stability of the closed-loop system is evaluated.

The impedance that human feels during the interaction with environment has critical importance in pHRI tasks. For instance, in a robotic assisted surgery, the control architecture for the interaction should ensure that the impedance of soft tissue (i.e. environment) is reflected to surgeon so that she/he can operate on patient more effectively. In such a case, the surgeon desires to feel the environment impedance (i.e. desired impedance) alone, and not the robot's impedance. Alternatively, in a different task, human may wish to move the robot in free space, where she/he does not desire to feel any dynamics coming from the robot. Therefore, depending on the task, a transparency metric can be defined based on the desired and reflected impedance to human.

\begin{enumerate}
\item For each parameter of the interaction controller, a range of values is chosen and discretized.

\item Bounds for the environment and human arm impedances (i.e. equivalent impedance) are selected based on the task.

\item A model for the robot is obtained.

\item A metric for transparency is defined and transparency is evaluated for each set of controller parameters.

\item Stability is evaluated for each set of controller parameters considering the bounds of the equivalent impedance.


\end{enumerate}
